A Kernel Mean Embedding Approach to Reducing Conservativeness in Stochastic Programming and Control

We apply kernel mean embedding methods to sample-based stochastic optimization and control. Specifically, we use the reduced-set expansion method as a way to discard sampled scenarios. The effect of such constraint removal is improved optimality and decreased conservativeness. This is achieved by solving a distributional-distance-regularized optimization problem. We demonstrated this optimization formulation is well-motivated in theory, computationally tractable and effective in numerical algorithms.

==> __latexindent_temp.tex <==
@article{erdougan2006ambiguous,
  title={Ambiguous chance constrained problems and robust optimization},
  author={Erdo{\u{g}}an, Emre and Iyengar, Garud},
  journal={Mathematical Programming},
  volume={107},
  number={1-2},
  pages={37--61},
  year={2006},
  publisher={Springer}
}

==> sec/method_moment.tex <==
To see this, by virtue of the fact that the equivalence of norms in finite
dimensional vector space. Hence, there exist \(c\) and \(C\) such that
\[
c\|\alpha\|_1 \leq \|\alpha\|_2\leq c\|\alpha\|_1.
\] Furthermore, as RKHS norm of the reduced-set embedding \[
\|\hat \mu^R_{x_{T}}\|_\mathcal H =   \|\sum_{i=1}^N \alpha^i \phi(x^i )\|_\mathcal H =\sqrt{\alpha^\top K\alpha}\leq \lambda_{\max}(K) \|\alpha\|_2\leq \lambda_{\max}(K)\cdot \|\alpha\|_1.
\] This makes evident that our optimization problem, effectively, is
minimizing an upper bound of the RKHS norm .

\subsubsection{Relation to generalized moment
problems.}

Our optimization problem \eqref{eq:l1} can in fact be interpret as the
generalize moment optimization problem. (cf.~Boyd) The intuitive idea of
moment problem is to 1) match the moments up to a certain order 2)
minimize any higher moments.

Similar to the above connection to RKHS regularization, if instead of
the \(l1\) norm, we penalize the RKHS norm
\(\|\hat \mu^R_{x_{T}}\|_\mathcal H\) associated with, say, \((p+1)\)-th
order polynomial kernel, we effectively have an generalized moment
optimization formulation defined in the sense of \[
\begin{aligned}
&\min _ {\alpha_i} & &\text{$(p+1)$-th order moment,}&\\
&s.t. & & \text{all moments lower than $p$-th match.}&
\end{aligned}
\] We make it evident as follows.
